Interpretable Neural Predictions with Differentiable Binary Variables

The success of neural networks comes hand in hand with a desire for more interpretability. We focus on text classifiers and make them more interpretable by having them provide a justification, a rationale, for their predictions. We approach this problem by jointly training two neural network models: a latent model that selects a rationale (i.e. a short and informative part of the input text), and a classifier that learns from the words in the rationale alone. Previous work proposed to assign binary latent masks to input positions and to promote short selections via sparsity-inducing penalties such as L0 regularisation. We propose a latent model that mixes discrete and continuous behaviour allowing at the same time for binary selections and gradient-based training without REINFORCE. In our formulation, we can tractably compute the expected value of penalties such as L0, which allows us to directly optimise the model towards a pre-specified text selection rate. We show that our approach is competitive with previous work on rationale extraction, and explore further uses in attention mechanisms.

==> fig/setup.tex <==
\begin{tikzpicture}
\node [] (w1) at (0,0)   {I};
\node [right of=w1] (w2) {loved};
\node [right of=w2] (w3) {this};
\node [right of=w3] (w4) {movie};

\node [above of=w1,node distance=5mm] (x1) {$Z_1$};
\node [above of=w2,node distance=5mm] (x2) {$Z_2$};
\node [above of=w3,node distance=5mm] (x3) {$Z_3$};
\node [above of=w4,node distance=5mm] (x4) {$Z_4$};

\node [above of=x1] (z1) {$z_1$};
\node [above of=x2] (z2) {$z_2$};
\node [above of=x3] (z3) {$z_3$};
\node [above of=x4] (z4) {$z_4$};

\node [above of=z1,node distance=5mm] (s1) {$0$};
\node [above of=z2,node distance=5mm] (s2) {$1$};
\node [above of=z3,node distance=5mm] (s3) {$1$};
\node [above of=z4,node distance=5mm] (s4) {$0$};

\draw[->,decorate, decoration=snake] (x1) -- (z1);
\draw[->,decorate, decoration=snake] (x2) -- (z2);
\draw[->,decorate, decoration=snake] (x3) -- (z3);
\draw[->,decorate, decoration=snake] (x4) -- (z4);

\node [right of=w4,node distance=20mm] (cw1) {loved this};
\node [above of=cw1,draw=tblue,fill=tblue!10] (classifier) {\small Classifier};
\node [above of=classifier] (result) {very positive};
\path[-stealth] (cw1) edge (classifier);
\path[-stealth] (classifier) edge (result);
\end{tikzpicture}
